Who Are All The Stochastic Parrots Imitating? They Should Tell Us!

Both standalone language models (LMs) as well as LMs within downstream-task systems have been shown to generate statements which are factually untrue. This problem is especially severe for low-resource languages, where training data is scarce and of worse quality than for high-resource languages. In this opinion piece, we argue that LMs in their current state will never be fully trustworthy in critical settings and suggest a possible novel strategy to handle this issue: by building LMs such that can cite their sources - i.e., point a user to the parts of their training data that back up their outputs. We first discuss which current NLP tasks would or would not benefit from such models. We then highlight the expected benefits such models would bring, e.g., quick verifiability of statements. We end by outlining the individual tasks that would need to be solved on the way to developing LMs with the ability to cite. We hope to start a discussion about the field's current approach to building LMs, especially for low-resource languages, and the role of the training data in explaining model generations.

==> tables/table1.tex <==
\begin{table}[t]
\centering
 \begin{tabular}{p{.95\columnwidth}} 
 \toprule
 \textbf{User:} Hi, ChatGPT! Can you explain the effects of drinking too little water to me, please?\\
 \midrule
 \textbf{ChatGPT:} Drinking too little water can cause dehydration, which can lead to a variety of symptoms and complications. Some common effects of dehydration include dry mouth, fatigue, dizziness, confusion, and dark-colored urine. Dehydration can also cause headaches, constipation, and decreased urine output. In severe cases, it can lead to more serious problems such as kidney stones, heat stroke, and even seizures or coma. It's important to drink enough water to stay properly hydrated and avoid these negative effects.\\
 \midrule
 \textbf{User:} Thanks! Where did you get this information from?\\
 \midrule
 \textbf{ChatGPT:} The information I provided is based on general knowledge and scientific studies on the effects of dehydration.  [...]\\
 \bottomrule
 \end{tabular}\caption{An actual conversation with ChatGPT on the effects of not drinking enough water. ChatGPT is unable to point the user to its sources and instead falls back to a general answer. We argue that ChatGPT and similar models should be able to direct the user to the sources of their information, which will have multiple benefits, such as quick verifiability of model statements.}
 \label{chat_gpt_conv}
\end{table}
